Computational-Statistical Tradeoffs at the Next-Token Prediction Barrier: Autoregressive and Imitation Learning under Misspecification

Next-token prediction with the logarithmic loss is a cornerstone of autoregressive sequence modeling, but, in practice, suffers from error amplification, where errors in the model compound and generation quality degrades as sequence length $H$ increases. From a theoretical perspective, this phenomenon should not appear in well-specified settings, and, indeed, a growing body of empirical work hypothesizes that misspecification, where the learner is not sufficiently expressive to represent the target distribution, may be the root cause. Under misspecification -- where the goal is to learn as well as the best-in-class model up to a multiplicative approximation factor $C\geq 1$ -- we confirm that $C$ indeed grows with $H$ for next-token prediction, lending theoretical support to this empirical hypothesis. We then ask whether this mode of error amplification is avoidable algorithmically, computationally, or information-theoretically, and uncover inherent computational-statistical tradeoffs. We show: (1) Information-theoretically, one can avoid error amplification and achieve $C=O(1)$. (2) Next-token prediction can be made robust so as to achieve $C=\tilde O(H)$, representing moderate error amplification, but this is an inherent barrier: any next-token prediction-style objective must suffer $C=\Omega(H)$. (3) For the natural testbed of autoregressive linear models, no computationally efficient algorithm can achieve sub-polynomial approximation factor $C=e^{(\log H)^{1-\Omega(1)}}$; however, at least for binary token spaces, one can smoothly trade compute for statistical power and improve on $C=\Omega(H)$ in sub-exponential time. Our results have consequences in the more general setting of imitation learning, where the widely-used behavior cloning algorithm generalizes next-token prediction.

==> section_imitation.tex <==
As a simple special case, if $\pistar$ is deterministic, then
combining \cref{prop:mle_finite}, leads to a guarantee on rollout
performance of the form $J(\pistar) - J(\pihat) \approxleq{}
R\cdot\frac{\log(\abs{\Pi}\delta^{-1})}{n}$. Under the ``dense-reward'' setting where $r_h\in\brk{0,1}$ for all $h\in\brk{H}$
so that $R=H$, this shows that behavior cloning can achieve constant
suboptimal with $\bigoh(H)$ examples, thereby evading the ``curse of
horizon'' known to plague other imitation learning algorithms (e.g.,
behavior cloning with other loss functions), under which $\bigom(H^2)$
sample complexity is observed \citep{ross2010efficient,ross2011reduction,ross2014reinforcement,
  rajaraman2020toward,rajaraman2021value,rajaraman2021provably,swamy2022minimax}. This
finding is salient because the curse of horizon has classically
been thought to blame for instabilities of imitation learning observed
in practice. %

per ,
also $\vepsmis$ represents irreducible error for rollout performance,
in the sense that any proper algorithm must have
$J(\pistar)-J(\pihat)\geq{}R\cdot\vepsmis^2$ for a worst-case reward
function. More importantly, the agnostic guarantee in
\cref{eq:hels-goal-intro} is sufficient to \emph{avoid the curse of
  horizon} for rollout performance: By , any algorithm that
satisfies \cref{eq:hels-goal-intro} achieves %
\[
  J(\pistar)-J(\pihat) \leq R\cdot{}(\Capx\cdot\vepsmis^2 + \vepsstatsn)
\]
when $\pistar$ is deterministic, meaning that even in the case of
dense rewards where $R=H$, the misspecification level is only scaled
by a \emph{linear} (as opposed to quadratic) factor in the horizon---so long as $\Capx$ itself is
independent of $H$.

